A Dynamic Temporal Logic for Quality of Service in Choreographic Models

We propose a framework for expressing and analyzing the Quality of Service (QoS) of message-passing systems using a choreographic model that consists of g-choreographies and Communicating Finite State machines (CFSMs). The following are our three main contributions: (I) an extension of CFSMs with non-functional contracts to specify quantitative constraints of local computations, (II) a dynamic temporal logic capable of expressing QoS, properties of systems relative to the g-choreography that specifies the communication protocol, (III) the semi-decidability of our logic which enables a bounded model-checking approach to verify QoS property of communicating systems.

==> aux.tex <==
%!TEX root = ./main.tex

\begin{definition}[Algebraic operators]\label{def:algop}
  An operator is said to be algebraic if it can be defined by a set of
  first order formula over the signature of the real closed
  fields. Alternatively, we can say that an algebraic operator is one
  that can be defined by algebraic equations, namely by using
  constants symbols, the basic arithmetic operators of the algebra
  $\_+\_$ and $\_ \cdot \_ $ and their opposites $\_-\_$, $\_/\_$,
  and their natural extension $\_^\_$ (exponentiation) and
  $\sqrt[\_]{\_}$ (root). See \cite[\S11.5]{hardy38} for an extensive
  discussion on algebraic equations and the mathematical properties of
  algebraic numbers.
\end{definition}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> auxrcf.tex <==
%!TEX root = ./main.tex

\begin{definition}[Ordered Field -- \cite{birkhoff65}(Sec.~2.1)]\label{def:ofield} 
Let $\Sigma_{\mathrm{field}} = \conf{\{0, 1\},\{+, \cdot\},\{=\}}$ and $\Gamma_{\mathrm{field}}$ the set containing the following formulae:
  $$
  \begin{array}{ll}
\text{(associativity)} & (\forall x, y, z)( x \cdot (y \cdot z) = (x \cdot y) \cdot z \land x + (y + z) = (x + y) + z)\\
\text{(commutativity)} & (\forall x, y)(x \cdot y = y \cdot x \land x + y = y + x)\\
\text{(identities)} & (\forall x)(x \cdot 1 = x \land x + 0 = x)\\
\text{(distributivity)} & (\forall x, y)(\forall z)x \cdot (y + z) = (x \cdot y) + (x \cdot z)\\
\text{($\cdot$ inverses)} & (\forall x)(x =  0 \lor ((\exists y) x \cdot y = 1))\\
\text{($+$ inverses)} & (\forall x)((\exists y) x + y = 0)
  \end{array}
  $$
Then, any model of the (first order) theory presentation $\conf{\Sigma_{\mathrm{field}}, \Gamma_{\mathrm{field}}}$ is said to be a \emph{field}.
%
An \emph{ordered field} is a field with a strict totally ordered
\footnote{Let $S$ be a set then $\leq \subseteq S \times S$ is a
  \emph{total order} if it satisfy the following conditions:
    \begin{inparaenum}[\itshape a\upshape)]
    \item Reflexivity: for all $a \in S$, $a = a$,
    \item Antisymmetry: for all $a, b, c \in S$, if $a \leq b$ and $b \leq a$ then $a = b$,
    \item Transitivity:  for all $a, b, c \in S$, if $a \leq b$ and $b \leq c$ then $a \leq c$, and
    \item Totality: for all $a, b \in S$, $a \leq b$ or $b \leq a$.
    \end{inparaenum}
Additionally, given $\leq \subseteq S \times S$ a total order, its associated \emph{strict total order} $< \subseteq S \times S$ is be defined by one of the following equivalent conditions:
    \begin{inparaenum}[\itshape a\upshape)]
    \item Reflexive reduction: for all $a, b \in S$, if $a \leq b$ and $\neg a = b$, then $a < b$, or
    \item $<$ is the complement of the converse of $\leq$: for all $a, b \in S$, if $\neg a \leq b$, then $a < b$.
    \end{inparaenum}
  } 
carrier set.
\end{definition}

Real-closed fields are ordered fields whose non-empty subsets all have a supremum.

\begin{definition}[Real-closed field -- \cite{birkhoff65}(Sec.~4.3)]\label{def:RCF}
  Given an ordered field with carrier $S$, its order
  $\leq \subseteq S \times S$ is \emph{Dedekind-complete} if every
  non-empty subset $S' \subseteq S$ with an upper bound in $S$ has a
  least upper bound (also called supremum) in $S$.
 
  Whenever $\leq$ is Dedekind-complete, the ordered field is said to
  be the \emph{real-closed field} (or a \emph{Dedekind-complete
    ordered field}).
\end{definition}

Intuitively, in Dedekind's own words, completeness implies that there
are not any \quo{gaps} in the real line, forcing the set to be
continuous.

 \begin{theorem}[Isomorphism of Real-closed fields \cite{erdos:am-3_61}(Thm.~2.1)]
   Under the continuum hypothesis, all hyper-real fields of power
   $\aleph_1$ are isomorphic.
 \end{theorem}

 \begin{corollary}
 \label{isomorphism}
 Given any two Dedekind-complete ordered fields with carrier sets $S$
 and $S'$ respectively, there exists a unique order-preserving field
 isomorphism from $S$ to $S'$.
 \end{corollary}

 In \cite{tarski:RM-109}, Tarski introduced what he called \emph{the system of elementary algebra}, his formalisation of the real numbers, as an ordered field (see \cite[Note~9]{tarski:RM-109}) also satisfying:
 \begin{inparaenum}[\itshape a\upshape)]
 \item an axiom stating that every positive number has a square root, and
 \item an axiom scheme stating that every polynomial of odd degree has, at least, one real root,
 \end{inparaenum}
 resulting in a first order theory that can be proved to be a Dedekind-complete ordered field \cite[Note~15]{tarski:RM-109}.
 \footnote{The proof of is obtained by first defining the topological completion of an ordered field $\mathit{F}$ by Dedekind cuts (denoted $\mathit{Dc}(\mathit{F})$) and then proving that, on the one hand:
 \begin{inparaenum}[\itshape a\upshape)]
 \item any polinomial of odd degree in an ordered field $\mathit{F}$, has a root in the topological completion $\mathit{Dc}(\mathit{F})$, and
 \item any element greater that $0$ in an ordered field $\mathit{F}$, has a square root in the topological completion $\mathit{Dc}(\mathit{F})$;
 \end{inparaenum}
 and, on the other hand, recalling that the topological completion $\mathit{Dc}(\mathit{F})$ of an ordered field $\mathit{F}$ satisfies the axioms of the system of elementary algebra.}.
 
 By \cref{isomorphism}, Tarski's system of elementary algebra is isomorphic to the real-closed field (see \cref{def:RCF}). Furthermore, Tarski proves that his system admits quantifier elimination \cite[Coro.~32]{tarski:RM-109} and, consequently, the existence of a decision procedure \cite[Thm.~37]{tarski:RM-109}.
 Tarski's decision procedure is of non-elementary complexity, meaning that given a problem of size $n$, it's complexity is not bound by any function of the form ${{{{2^2}^\cdot}^\cdot}^\cdot}^n$. In \cite{monk+:manuscript74}, Monk provided an elementary complexity algorithm quantifier elimination. In \cite[Corollary to Thm.~1]{davenport:jsc-5_1} Davenport and Heintz proved that quantifier elimination for real-closed field is doubly exponential in the size of the problem. Algorithms of such a complexity were provided by Collins in \cite{collins:atfl75}, and Monk in \cite{monk+:phdthesis}, independently. Later, in \cite{ben-or:jcss-32_2}, Ben-Or et. al proposed a different algorithm running in exponential space or parallel exponential time in the size of the problem.\\


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> introduction.tex <==
%!TEX root = ./main.tex

The way in which software systems are constructed and deployed has radically changed over the last decades. Nowadays software artifact are no longer monolithic constructions running in isolation. Instead, they can be though of as cooperating components, communicating on an adequate environment to perform its execution. Even more, there is a rapidly increasing number of software systems that are conceived, from its design stage, as a set of participants executing over globally available computational resources, and interacting with each other over existing communication infrastructure, in a distributed way in order to fulfill a collective goal.

There is big body of work versing on the problem of formalising the
communicating behaviour of distributed systems. Among those languages
choreographies stand out. Choreographic models of advocate a
\emph{global view} and a \emph{local view}.
%
The former is a high-level description of the interactions among
components that abstracts away some aspects in order to offer a
holistic understanding of the communication behaviour of the
system.
%
The latter view is a description of each component in isolation.
%
% They can be described both from a global point of view (see \eg~\cite{denielou:esop12} or from a local point view (i.e., the standpoint of each individual component) (see \eg~\cite{brand:jacm-30_2}, and for which there exists associated analysis methods like synthesis of \emph{Global graphs} from \emph{Communicating Finite State Machines} (CFSMs) \cite{lange:popl15} that can be applied in order to determine realisability free from communication errors or conformance of a component's behaviour to a protocol \cite{vissani:places15}.

With the flourishing of ubiquitous computing and the emergence of more
dynamic computing paradigms such as Cloud/Fog/Edge Computing, Service
Oriented Computing and, what is sometimes referred to as, the API's
economy~\cite{dwasl16,apiIBM}, reasoning about the QoS of the
components has become a key issue in the design and execution of
distributed systems.
%
In previous work~\cite{martinezsune:coordination19} we have proposed an automatically analysable specification language for QoS where contracts are captured as constraints over quantitative attributes of interest (\eg~computation time required, storage required, waiting time, cost, etc.). Such specifications can be thought of as logical characterisations of the admisible values of the quantitative attributes of the software component along its executions.

When software components are observed from the standpoint of their communication behaviour (\eg~when they are specified through the use of languages like CFSMs) we access a different, one could say more internal, view of how the computation is performed. From this viewpoint a component's computation can be rationalised along a run whose states correspond to states of the CFSM, and describe bits of the computation, linked by the communication actions. Therefore, we can naturally extend the language of the CFSMs by attaching QoS constracts to the states, describing the cost associated to the computation performed in them.

\eMcomm{
  should we claim that this is the first framework of behavioural types with QoS
}{Our main contributions are as follows.}

\begin{itemize}
\item A modelling language to express QoS attributes of components.
  %
  The language is straightforwardly attained by the states of CFSMs
  with constraints specifying QoS aspects of local computations.
  %
  This design decision assumes that there is no control on communication
  infrastructure.
  %
  More precisely, QoS aspects related to how communications are
  realised are not under the control of applications' designers.
  %
  Instead, designers have control on local computation, thus
  suggesting that QoS constraints are naturally associated to states
  of CFSMs.
  %
  We decided to adopt real-closed fields to represent QoS values;
  besides being a complete and decidable abstract formalisation of the
  real numbers, real-closed fields are instrumental for a smooth
  definition of our framework.
  % %
  % In particular, real-closed fields (and their extensions
  % to express QoS constraints) can be conveniently defined as
  % presentations of first-order theories.
\item A logical language for describing QoS properties of interest of
  communicating systems.
  %
  Our logic, dubbed $\QL$, is inspired by \emph{Propositional Dynamic
	 Linear Temporal Logic} (DLTL) \cite{henriksen:apal-96_1_3}.
  %
  A distinct characteristic of $\QL$ is that it indexes temporal
  modalities with \emph{g-choreographies}~\cite{tuosto:jlamp-95}, a
  model of global views of choregraphies, in order to predicate on QoS
  properties of the whole system.
  %
  Noteworthy, we could not directly use $\DLTL$ for our
  purposes.
  %
  This is due to two limitations shortcomings.
  \begin{inparaenum}[1)]
  \item The satisfiability of a $\DLTL$ formula relies on the
	 prefixes of runs being checked to belong to the language of the
	 regular expressions.
	 %
	 In our case, this is not enough; as it will become clear in
	 \cref{sec:logic} (cf. \cref{def:aggregation-function} and
	 \cref{def:ql-semantics}), in our proposal, satisfaction will
	 require collecting information along the prefix of \emph{maximal}
	 runs.
  \item In $\DLTL$ modalities are indexed by regular
	 expressions over atomic actions.
	 %
	 In our case, this would mean to use an alphabet of output and
	 input actions.
	 %
	 However, global views of choregraphies (such as g-choreographies)
	 hinge on \emph{interactions}, an abstraction to represent
	 handshakes between a sender an a receiver.
	 %
	 Also, such interactions are then realised asynchronously thus
	 breaking the atomicity.
  \end{inparaenum}
\item \eMcomm{}{I'll expand this} A decision procedure for checking
  satisfiability of QoS properties by a communicating system.
\end{itemize}
These contributions collectively constitute a framework achieving what
we believe is a crucial need of modern distributed computational
models like those mentioned before.

The paper is organised as follows: in Sec.~\ref{sec:pre} we provide
the formal definitions regarding communicating systems and the
specification of quantitative attributes that will use in the rest of
the paper; in Sec.~\ref{sec:QoS-choreo} we present the main
contribution of the paper, a QoS extension of communicating machines
and a logical language to express QoS properties, together with an
analysis algorithm presented in \cref{sec:analysis}. Finally, in
Sec.~\ref{sec:conclu} we draw some conclusions and point out some
further lines of research.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> methodology.tex <==
% !TEX root = ./main.tex

% We now present our methodology for the design of QoS-aware distributed
% systems.
%
Our methodology aims to specify and analyse QoS of the overall system
starting from guarantees on the QoS of components.
%
We describe the methodology on a multi-party variant of our running
example.
%
Inspired in the OAuth authentication protocol \cite{rfc6749}, the idea is that before 
contacting the POP server $\p[s]$ the client
$\p[c]$ should get an authentication token from an authentication
server $\p$.
%
This is captured by the g-choreography $\gpop{pop'}$ below:
\begin{align*}
  \gpop{pop'} & = \gseq[][{\gint[][c][cred][a]}][{ (\gcho[][ { \gseq[][{\gint[][a][token][c]}] [{\gpop{pop''}}] } ][ {\gint[][a][error][c]} ]) }]
  \\
  \gpop{pop''} & = \gcho[][ {\gseq[][ {\gseq[][{\gint[][c][helo][s]}][{\gint[][c][token][s]}]} ] [ ({ \gcho[][ {\gint[][s][fail][c]} ][{\gpop{helo'}}] }) ] } ][{\gpop{quit}}]
  \\
  \gpop{helo'} & = \gcho[][{\gseq[][{\gint[][s][int][c]}][({\grec[][\gpop{read}]}]}][{\gpop{quit}})]
\end{align*}
where $\gpop{read}$, $\gpop{retr}$, and $\gpop{quit}$ are as in
\cref{ex:gpop}.

The first step of our methodology requires to specify each CFSM.  When
analysing an actual implementation, CFSMs could be extracted from code
implementing the components or designed directly.
%
Alternatively, CFSMs can be obtained by \emph{projecting} a
g-choreography specifying the protocol.
%
For example, we can use ChorGram to project the CFSMs shown below, from the g-choreograpgy $\gpop{pop'}$ presented above:
\begin{align*}
    \begin{tikzpicture}[node distance=.3cm and 1cm, every node/.style={scale=1,transform shape}]
        \node (d) at (0,0) {};
        \node[cnode,right= .3cm of d] (0) {};
        \node[cnode,right = of 0] (1) {};
        \node[cnode,above right = of 1] (2) {};
        \node[cnode,below right = of 1] (3) {};
%
        \path[line] (d) -- (0);
        \path[line] (0) edge node[below]{$\ain[c][a][cred]$} (1);
        \path[line] (1) edge[sloped] node[above]{$\aout[a][c][token]$} (2);
        \path[line] (1) edge[sloped] node[below]{$\aout[a][c][error]$} (3);
%
        \node[draw,text width=1.8cm] at (0.5,1) {$\ptp[A]$: Auth. server};
    \end{tikzpicture}
% \qquad
    \begin{tikzpicture}[node distance=1cm and 1cm, every node/.style={scale=1,transform shape}]
        \node (d) at (0,0) {};
        \node[cnode,right= .3cm of d] (0) {};
        \foreach \s/\t in {0/1,1/1b,1b/2,2/3,3/4,4/5,5/6} {
           \node (\t) [cnode, right = of \s] {};
        }
        \foreach \s/\l/\t in {0/\ain[c][s][helo]/1,1/\ain[s][c][token]/1b,1b/\aout[s][c][int]/2,2/\ain[c][s][read]/3,3/\aout[s][c][size]/4,4/\ain[c][s][retr]/5,5/\aout[s][c][msg]/6} {
           \path[line,sloped] (\s) edge node[below]{$\l$} (\t);
        }
        \node[cnode,above = of 0] (7) {};
        \node[cnode,right = of 7] (8) {};
        \node[cnode,below = of 1b] (9) {};
        %
        \path[line] (d) -- (0);
        \path[line] (6) edge[bend left=-35] node[below]{$\ain[c][s][ack]$} (2);
        \path[line] (0) edge node[left]{$\ain[c][s][quit]$} (7);
        \path[line] (2) edge node[left]{$\ain[c][s][quit]$} (7);
        \path[line] (4) edge[sloped] node[above]{$\ain[c][s][quit]$} (7);
        \path[line] (7) edge node[above]{$\aout[s][c][bye]$} (8);
        \path[line] (1b) edge node[below right]{$\aout[s][c][fail]$} (9);
%
        \node[draw,text width=1.8cm] at (6,1.2) {$\ptp[S]$: POP server};
    \end{tikzpicture}
\\
    \begin{tikzpicture}[node distance=1cm and 1.1cm, every node/.style={scale=1,transform shape}]
        \node (d) at (0,0) {};
        \node[cnode,right= .3cm of d] (auth0) {};
        \node[cnode,right= of auth0] (auth1) {};
        \node[cnode,right= of auth1] (0) {};
        \node[cnode,above= of auth1] (authFail) {};
%        
        \foreach \s/\t in {0/1,1/1b,1b/2,2/3,3/4,4/5,5/6} {
           \node (\t) [cnode, right = of \s] {};
        }
        \foreach \s/\l/\t in {0/\aout[c][s][helo]/1,1/\aout[c][s][token]/1b,1b/\ain[s][c][int]/2,2/\aout[c][s][read]/3,3/\ain[s][c][size]/4,4/\aout[c][s][retr]/5,5/\ain[s][c][msg]/6} {
           \path[line,sloped] (\s) edge node[below]{$\l$} (\t);
        }
        \node[cnode,above = of 0] (7) {};
        \node[cnode,right = of 7] (8) {};
        \node[cnode,below = of 1b] (9) {};
%        
        \path[line] (d) -- (auth0);
        \path[line] (auth0) edge node[below]{$\aout[c][a][cred]$} (auth1);
        \path[line] (auth1) edge node[left]{$\ain[a][c][error]$} (authFail);
        \path[line] (auth1) edge node[below]{$\ain[a][c][token]$} (0);
        \path[line] (6) edge[bend left=-35] node[below]{$\aout[c][s][ack]$} (2);
        \path[line] (0) edge node[left]{$\aout[c][s][quit]$} (7);
        \path[line] (2) edge node[left]{$\aout[c][s][quit]$} (7);
        \path[line] (4) edge[sloped] node[above]{$\aout[c][s][quit]$} (7);
        \path[line] (7) edge node[above]{$\ain[s][c][bye]$} (8);
        \path[line] (1b) edge node[below right]{$\ain[s][c][fail]$} (9);
%
        \node[draw,text width=1.8cm] at (0.5,1) {$\ptp[C]$: POP client};
    \end{tikzpicture}
    % \caption{Communicating system for POP with authentication.}
\end{align*}
In this case, since $\gpop{pop'}$ is well-formed,
the machines are correct by construction.
%
Otherwise, we can use ChorGram to check multiparty
compatibility~\cite{lange:gay17}, which indicates if the components
will be able to interact successfully.
%
In such case, ChorGram also computes a g-choreography that
faithfully represent the behaviour of the CFSMs.

The second step is to identify QoS attributes
and assign QoS specifications to CFSMs.
%
As for POP, our  QoS attributes are time, monetary cost, and
memory (together with the same aggregation operators used so far).
%
The assignement of QoS specification to CFSMs is crucial; the quality
of the analysis strongly depends on this step: the more accurate QoS
specifications are the more accurate the results of the analysis will
be.
%
Identifying QoS specifications is application-dependent.
%
For instance, some domains (such as on-board software in autonomous
vehicles or in the aerospace domain) have rather precise bounds on
computations on which critical behaviour relies.
%
In other case, QoS specifications can be obtained by profiling
components, from statistical inference from the observation on
their execution, or can be based on experts' knowledge.

For the sake of the presentation, let
$\Gamma_{\constset[Q]_{\mathrm{Chk}}} = \{ t \leq 5, c = 0.5, m = 0
\}$ be one of our QoS specification. Following the rationale already 
used in \cref{ex:qosspec}, $\Gamma_{\constset[Q]_{\mathrm{Chk}}}$ 
models the computational costs of checking the integrity of a received
message. Therefore it would be mapped to \p[c] right 
after receiving a message, as the following fragment of the machine \p[c] shows:
% \begin{center}
\begin{align*}
    \begin{tikzpicture}[node distance=1cm and 1.3cm, every node/.style={scale=1,transform shape}, every label/.style={color=blue,fill=yellow!10,scale=.7}]
        \def\chk{\Gamma_{\constset[Q]_{\mathrm{Chk}}}}
        \node[cnode] (0) at (0,0) {};
        \node[cnode, left= of 0] (-1) {};
        \node[left= of -1] (-2) {};
        \node[cnode,right= of 0, label=$\chk$] (1) {};
        % \node[label={above:$\{ t \leq 5, m = 0 \}$}] (1) {$\aQzero$};
        \node[right= of 1] (2) {};
%
        \path (-2) -- node[auto=false]{\ldots} (-1);
        \path[line] (-1) edge node[below]{$\aout[c][s][retr]$} (0);
        \path[line] (0) edge node[below]{$\ain[s][c][msg]$} (1);
        \path (1) -- node[auto=false]{\ldots} (2);
    \end{tikzpicture}
\end{align*}
% \end{center}
If this procedure is repeated for every state in every machine then
 we have a complete QoS-extended system, a comprehensive QoS aware 
 model of the behaviour of the system.
The focus now shifts to the properties we would like our system to
satisfy.
%
Suppose we would like to check a specific relation between the
monetary cost for the client $\p[c]$ to download messages, and the
execution time; for instance, let $\psi$ be the constraint
$t > 1 \implies c < 10 t$ stating that, whenever the aggregated time
is above one second, the monetary cost is lower than the aggregated
time multiplied by ten.
%
The structure of our property is then as follows
$\gqosprop = [\aG] \psi$ (recall that $\gqosprop$
is equivivalent to
$\neg\ (\top\ \until[\aG]\ \neg\psi)$).
%
But what should the index $\aG$ be in $\gqosprop$?
%
We can determine $\aG$ by inspecting the g-choreography $\gpop{pop'}$
above, in order to identify the point(s) of the protocol where \p[c] downloads
messages; this yields
\begin{align*}
  \aG = &\ \gint[][c][cred][a];
			 \gint[][a][token][c];
			 \gint[][c][helo][s];
			 \gint[][c][token][s];
			 \gint[][s][int][c];
			 \grec[][\aG_1]
\end{align*}
where
$\aG_1 = \gint[][c][read][s]; \gint[][s][size][c];
\gint[][c][retr][s]; \gint[][s][msg][c]; \gint[][c][ack][s]$.
%
In words, $\aG$ above characterises runs where, after successful
authentication, \p[c] iteratively downloads messages from \p[s].

Formula $\gqosprop$ can be verified with a bounded model checking approach
(cf. \cref{sec:analysis}).
%
This approach requires to first choose a bound $k$ for the number of
iterations in $\aG$ in order to obtain a formula $\gqosprop'$ in $\QL^-$.
%
A natural choice for our scenario is to let $k$ be an upper bound on
the number of messages received by $\p[c]$.
%
Then, we can feed \textsc{qSat} with the formula $\neg\gqosprop'$,
together with the QoS extended communicating system. The analysis will
tell whether $\neg\gqosprop'$ is satisfiable or not. If
$\neg\gqosprop'$ is not satisfiable we have the guarantee that every
run of the system, up to $k$ messages received by $\p[c]$, satisfies
the formula $\gqosprop$. At this point we might choose to increase the
bound $k$ and repeat the procedure in order to have guarantees for
larger numbers of iterations of the g-choreography. If, on the other
hand, $\neg\gqosprop'$ is satisfiable, we can be certain that the
system violates formula $\gqosprop$ because there exists an execution
that serves as a witness of such a violation.  Finally, after that
verdict, there are different possible courses of action.  We might
weaken the QoS constraint $\psi$ in order to check a looser constraint
or we might modify the QoS specifications assigned to the states of
the components of the systems, aiming at strengthening them in order
to satisfy $\gqosprop$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> qsat.tex <==
\begin{algorithm}[H]
% \caption{Decision procedure for the satisfiability of $\QL^-$ formulae}
% \label{alg:check}
\DontPrintSemicolon
\SetAlgoLined
\KwData{$\gqosprop$ QoS formula, $\aCS$ communicating system, $\pi \in \Delta_{\aCS}$  run of $\aCS$}
\KwResult{A set of runs: $\emptyset \iff \aCS \models \gqosprop$}
\SetKwFunction{check}{\textsc{qSat}}
\SetKwFunction{traceOf}{\textsc{TraceOf}}
\check{$\gqosprop,\aCS,\pi$}:\\
\lnl{1}\lIf{$\gqosprop \in \qosspecs$}{
  \Switch{\texttt{SMT}($\aggfn (\pi), \gqosprop$)}{
	 \lCase{\textbf{true}}{\Return{$\emptyset$}}
    \lCase{\textbf{false}}{\Return{$\{\pi\}$}}
  }
}
\Switch{$\gqosprop$}{
  \lnl{2}\lCase{$\neg\gqospropb$}{
	 \Switch{$\gqospropb,\aCS,\pi$}{
		\lCase{$\emptyset$}{\Return{$\{\pi\}$}}
		\lCase{\textbf{otherwise}}{\Return{$\emptyset$}}
	 }
  }
  \lnl{3}\lCase{$\gqospropb \lor \gqospropb'$}{
	 \Switch{\check{$\gqospropb,\aCS,\pi$}}{
		\lCase{$\emptyset$}{\check{$\gqospropb',\aCS,\pi$}}
		\lCase{\textbf{otherwise}}{\Return{$\{\pi\}$}}
	 }
  }
  \Case{$\gqospropb\ \mathcal{U}^\aG\ \gqospropb'$}{
	 \lnl{4}\lIf{\check{$\gqospropb',\aCS,\pi$} == $\emptyset$}{\Return{$\emptyset$}}
	 \Else{
		\lnl{5}\ForEach{$\aConf \TRANSS{\al} \aConf'$ on $\aCS$}{
		  \lnl{6}\lIf{\check{$\gqospropb,\aCS,\pi$} == $\emptyset$
			 \textbf{\emph{and}}
			 \traceOf{$\pi \cdot \aConf \TRANSS{\al} \aConf'$}
			 $\in \mathcal{L}(\aG)$}{
			 \check{$\gqospropb\ \mathcal{U}^\aG\ \gqospropb',\aCS, \pi \cdot \aConf \TRANSS{\al} \aConf'$}}
		}
	 }
  }
  \lnl{8}\lCase{$\top$}{\Return{$\emptyset$}}
  \lnl{9}\lCase{$\bot$}{\Return{$\{\pi\}$}}
}
\end{algorithm}


\begin{algorithm}[H]
% \caption{Decision procedure for the satisfiability of $\QL^-$ formulae}
% \label{alg:check}
\DontPrintSemicolon
\SetAlgoLined
\KwData{$\gqosprop$ QoS formula, $\aCS$ communicating system, $\pi \in \Delta_{\aCS}$  run of $\aCS$}
\KwResult{A singleton with a witness that $\aCS\models \gqosprop$ (if any, otherwise $\emptyset$)}
\SetKwFunction{check}{\textsc{qSat}}
\SetKwFunction{traceOf}{\textsc{TraceOf}}
\check{$\gqosprop,\aCS,\pi$}:\\
\lnl{1}\lIf{$\gqosprop \in \qosspecs$}{
  \Switch{\texttt{SMT}($\aggfn (\pi), \gqosprop$)}{
	 \lCase{\textbf{true}}{\Return{$\{\pi\}$}}
    \lCase{\textbf{false}}{\Return{$\emptyset$}}
  }
}
\Switch{$\gqosprop$}{
  \lnl{2}\lCase{$\neg\gqospropb$}{
	 let tmp = \check{$\gqospropb,\aCS,\pi$} 
	 \Switch{tmp}{
		\lCase{$\emptyset$}{\Return{$\{\pi\}$}}
		\lCase{\textbf{otherwise}}{\Return{$\emptyset$}}
	 }
  }
  \lnl{3}\lCase{$\gqospropb \lor \gqospropb'$}{
	 let tmp = {\check{$\gqospropb,\aCS,\pi$}}
	 \Switch{tmp}{
		\lCase{$\emptyset$}{\check{$\gqospropb',\aCS,\pi$}}
		\lCase{\textbf{otherwise}}{\Return{tmp}}
	 }
  }
  \Case{$\gqospropb\ \mathcal{U}^\aG\ \gqospropb'$}{
	 \lnl{4}\lIf{\check{$\gqospropb',\aCS,\pi$} $\neq \emptyset$}{\check{$\gqospropb',\aCS,\pi$}}
	 \Else{
		\lnl{5}\ForEach{$\aConf \TRANSS{\al} \aConf'$ on $\aCS$}{
		  \lnl{6}\lIf{{\check{$\gqospropb,\aCS,\pi$}} $\neq \emptyset$
  \textbf{\emph{and}}
			 \traceOf{$\pi \cdot \aConf \TRANSS{\al} \aConf'$}			 $\in \mathcal{L}(\aG)$
}{	 let tmp = 			 \check{$\gqospropb\ \mathcal{U}^\aG\ \gqospropb',\aCS, \pi \cdot \aConf \TRANSS{\al} \aConf'$}
			 \lIf{\\tmp \neq $\emptyset$}{\Return{tmp}}
}{
		  }
		}
	 }
  }
  \lnl{8}\lCase{$\top$}{\Return{$\{\pi\}$}}
  \lnl{9}\lCase{$\bot$}{\Return{$\emptyset$}}
}
\end{algorithm}
\end{document}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rcf.tex <==
%!TEX root = ./main.tex
%c
% Real numbers are natural candidates to express quantitative attributes
% of a software artefact.
% %
% We adopt \emph{real-closed fields} (RCFs), the formalisation of the
% first-order theory of the real numbers, as a foundations for QoS
% values.
% %
% The main reason for this choice is that theories extending the RCFs
% are decidable, providing effective means for analysis.
%
Hereafter, we assume that the reader is acquainted with the
language of first-order predicate logic with equality
($\mathit{FOL}_=$), its semantics and associated
calculus~\cite{smullyan68,enderton72}.
%
We fix a denumerable set of variable symbols $\varset$ and an arbitrary
signature $\Sigma = \conf{\constset, \mathtt{F}, \mathtt{P}}$
consisting of the constant, function, and predicate symbols.
%
A first-order logic over $\Sigma$ is defined as usual.
%
Let $\termalg$ and $\formulas$ respectively denote the set of terms
and formulae over $\Sigma$ and $\varset$.

A \emph{$\Sigma$-interpretation} is a structure
$\mathcal{I} = \conf{S, \{\overline{c}\}_{c \in \constset},
  \{\overline{f}\}_{f \in \mathtt{F}}, \{\overline{p}\}_{p \in
	 \mathtt{P}}}$ assigning meaning to the symbols in $\Sigma$
respectively as elements of the \emph{carrier set} $S$, as functions,
and as predicates over $S$.
%
A \emph{model} $\mathcal{M}$ consists of a pair
$\conf{\mathcal{I}, v}$ where $\mathcal{I}$ is a
$\Sigma$-interpretation and $v: \varset \to S$ is a \emph{valuation}
assigning meaning to variables over the carrier set of
$\mathcal{I}$.
%
We let $\modelsclass$ to be the class of models for $\Sigma$,
$\varset$ and $\models \subseteq \modelsclass \times \formulas$ the
satisfaction relation recursively defined on the structure of the
formula as usual.
%
The entailment relation
$\vdash \subseteq 2^{\formulas} \times \formulas$ can be formalised
through axioms and rules
% as any complete calculus of choice
(see e.g.,~\cite{hilbert50}, \cite[Sec.~II]{gentzen:apq-1_4}, or \cite[Sec.~2.4]{enderton72}).
%
%Fixed an arbitrary signature $\Sigma = \conf{\constset, \mathtt{F}, \mathtt{P}}$ consisting of the constant, function, and predicate symbols and given a denumerable set of variable symbols $\varset$, an first-order logic over $\Sigma$ is defined as usual; let $\termalg$ and $\formulas$ to respectively be the set of terms and formulae over $\Sigma$ and $\varset$.
%
%A \emph{$\Sigma$-interpretation} is a structure $\mathcal{I} = \conf{S, \{\overline{c}\}_{c \in \constset}, \{\overline{f}\}_{f \in \mathtt{F}}, \{\overline{p}\}_{p \in \mathtt{P}}}$, where the set $S$ is the \emph{carrier set} such that:
%\begin{inparaenum}[i)] 
%\item $\overline{c} \in S$, for all $c \in \constset$, 
%\item $\overline{f}: S^{\mathit{arity(f)}} \to S$, for all $f \in \mathtt{F}$, and
%\item $\overline{p} \subseteq S^{\mathit{arity(p)}}$ for all $p \in \mathtt{P}$,
%\end{inparaenum}
%assigning meaning to the symbols as elements, functions and predicates over $S$, respectively.
%
%Given a signature $\Sigma$, a \emph{model} $\mathcal{M}$ consists of a
%pair $\conf{\mathcal{I}, v}$ where $\mathcal{I}$ is a
%$\Sigma$-interpretation and $v: \varset \to S$ is a \emph{valuation}
%assigning meaning to variables over the carrier set $S$ of
%$\mathcal{I}$.
%
%The class of models for $\Sigma, \varset$ is denoted as $\modelsclass$.
%
%The satisfaction relation between models and formulae $\models \subseteq \modelsclass \times \formulas$ is defined recursively on the structure of the formula as usual.
%
%The entailment relation $\vdash \subseteq 2^{\formulas} \times \formulas$ can be formalised through the axioms and rules of any complete calculus of choice (see, for instance, \cite[Drittes Kapitel]{hilbert28} for a Hilbert-style calculus, \cite[Sec.~II]{gentzen:apq-1_4} for a natural deduction calculus and \cite[Sec.~2.4]{enderton72} for a classical calculus, among others, and \cite{troelstra96} for a more comprehensive presentation of them).
%
A set of formulae $\Gamma \in 2^{\formulas}$ is a \emph{first-order theory} if
$\Gamma$ is closed under deduction (i.e., $\Gamma \vdash \alpha$
implies $\alpha \in \Gamma$ for all $\alpha \in \formulas$).
%
A \emph{(first-order) theory presentation over $\Sigma$} is a pair
$\conf{\Sigma, \Gamma}$ where $\Gamma \subseteq \formulas$.
%
The notion of model extends naturally to theory presentations:
$\mathcal{M} \models \conf{\Sigma, \Gamma}$ iff
$\mathcal{M} \in \modelsclass$ and $\mathcal{M} \models \varphi$, for
all $\varphi \in \Gamma$.

Let $\Sigma_{\mathrm{field}}$ be the signature $\conf{\{0, 1\},\{+, \cdot\},\{=\}}$.
%
An ordered field is a first-order theory presentation
$\conf{\Sigma_{\mathrm{field}}, \Gamma_{\mathrm{field}}}$ where
$\Gamma_{\mathrm{field}}$ are the field axioms 
% (cf.~\cref{def:ofield}
% in \cref{sec:auxrcf}).
%
Real-closed fields are ordered fields whose non-empty subsets all have
a supremum.% (cf.~\cref{def:RCF} in \cref{sec:auxrcf}).
%
In \cite{tarski:RM-109}, Tarski introduced \emph{the system of
  elementary algebra} as a first-order theory of real numbers for
which he proved that:
\begin{inparaenum}[a)]
\item it is a real-closed field \cite[Note~15]{tarski:RM-109}, and
\item there exists a decision procedure \cite[Thm.~37]{tarski:RM-109}.
\end{inparaenum}
Furthermore, all real-closed fields are isomorphic
\cite{erdos:am-3_61}(Thm.~2.1). 
% See \cref{sec:auxrcf} for a more
% detailed account on the theoretical aspects of the real-closed
% fields.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> sem.tex <==
\anote{Review integration of text, examples and formal definitions in this section.}

The semantics of g-choreographies has been defined in
\cite{tuosto:jlamp-95} in terms of \emph{pomsets}
\cite{pratt:ijpp-15_1} labelled over
the set of \emph{communication actions}
$\lset = \lset^!  \cup \lset^?$.


Basically, the semantics $\gsem$ of a g-choreography $\aG$ is a set of
pomsets representing the causal relations among communication events
in $\aG$.
%
Due to space limitations, we give only an intuitive account of the
semantics 
% (
	% a compact technical presentation is in
% \cref{sec:sem}; 
(the reader is referred
to~\cite{tuosto:jlamp-95} for more details).
%
For instance, the semantics of an interaction is just a partial order
such that the event corresponding to the output precedes the one
corresponding to the input while the semantics of a parallel $\gpar[]$
composition is obtained by taking the disjoint unions of each pomset
in $\gsem$ and each one in $\gsem[\aG']$.
%
It is a straightforward observation that the semantics of $\star$-free
g-choreographies is a finite disjoint union of finite pomset.
%
We illustrate this intuition in the next example.
%
\begin{example}[An excerpt of POP's semantics]\label{ex:sem}
  The semantics of $\gpop{quit}$ in~\cref{ex:gpop} and of
  $\aG = \gint[][c][helo][s]; \gint[][s][int][c]$ (representing a
  possible initial run of POP) are the singletons
  \begin{align*}
	 \begin{array}[c]{c@{\qqand}c}
		\gsem[\gpop{quit}] = \left\{\pomset[1]{
		\node (1) {$\aout[c][s][quit]$};
		\node[right = of 1] (2) {$\ain[c][s][quit]$};
		\node[below = of 1] (3) {$\ain[s][c][bye]$};
		\node[below = of 2] (4) {$\aout[s][c][bye]$};
		%
		\path[draw,->] (1) -- (2);
		\path[draw,->] (4) -- (3);
		\path[draw,->] (1) -- (3);
		\path[draw,->] (2) -- (4);
		}
		\right\}
		&
		\gsem = \left\{\pomset[1]{
		\node (1) {$\aout[c][s][helo]$};
		\node[right = of 1] (2) {$\ain[c][s][helo]$};
		\node[below = of 1] (3) {$\ain[s][c][int]$};
		\node[below = of 2] (4) {$\aout[s][c][int]$};
		%
		\path[draw,->] (1) -- (2);
		\path[draw,->] (4) -- (3);
		\path[draw,->] (1) -- (3);
		\path[draw,->] (2) -- (4);
		}
		\right\}
	 \end{array}
  \end{align*}
  where we represent pomsets as (a variant\footnote{Edges of Hasse
	 diagrams are usually not oriented; here we use arrows so to draw
	 order relations between events also horizontally.} of) Hasse
  diagrams of the immediate predecessor relation enclosed in square
  brackets.\anote{R2: ‘Hasse diagrams of the immediate predecessor relation’ - please explain more, this sentence requires some background notion that is out of context here.}
  %
  Accordingly, we have $\gsem[{\gcho[][\gpop{quit}][\aG]}] = \gsem[\gpop{quit}] \cup \gsem[\aG]$
  while
  \begin{align*}
	 \gsem[{\gpar[][\gpop{quit}][\aG]}] =
	 \left\{\pomset[1]{
	 \node (1) {$\aout[c][s][helo]$};
	 \node[right = of 1] (2) {$\ain[c][s][helo]$};
	 \node[below = of 1] (3) {$\ain[s][c][int]$};
	 \node[below = of 2] (4) {$\aout[s][c][int]$};
	 %
	 \path[draw,->] (1) -- (2);
	 \path[draw,->] (4) -- (3);
	 \path[draw,->] (1) -- (3);
	 \path[draw,->] (2) -- (4);
	 %%
	 \node[right = 1cm of 2] (a) {$\aout[c][s][quit]$};
	 \node[right = of a] (b) {$\ain[c][s][quit]$};
	 \node[below = of a] (c) {$\ain[s][c][bye]$};
	 \node[below = of b] (d) {$\aout[s][c][bye]$};
	 %
	 \path[draw,->] (a) -- (b);
	 \path[draw,->] (d) -- (c);
	 \path[draw,->] (a) -- (c);
	 \path[draw,->] (b) -- (d);
	 }
	 \right\}
  \end{align*}
  formalising that the communications in $\gpop{quit}$ and those in
  $\aG$ may occur in any order since they are not related by any
  causal dependency.
  %
  \finex
\end{example}

The \emph{linearisations} of a pomset $\apom$ is the sequence of the communication
action obtained by a permutation of the events of $\apom$ that
preserves the causality relation of $\apom$.
%
For instance, the only possible linearisation of the pomset in
$\gsem[\gpop{quit}]$ (cf. \cref{ex:sem}) is the sequence
$\aout[c][s][quit]\ \ain[c][s][quit]\ \aout[s][c][bye]\
\ain[s][c][bye]$ while
$\aout[c][s][quit]\ \aout[s][c][bye]\ \ain[c][s][quit]\
\ain[s][c][bye]$ is not a linearisation because it violates the causal
dependency between $\aout[s][c][bye]$ and $\ain[c][s][quit]$.
%
The \emph{language} of $\aG$ is the set $\rlang[\aG]$ of sequences of
linearisations of a pomsets in $\gsem$.

\begin{definition}
  A labelled partially-ordered set (lposet) is a triple
  $(\eset, \leq, \alf)$, with $\eset$ a set of events,
  $\leq \subseteq \eset \times \eset$ a reflexive, anti-symmetric, and
  transitive relation on $\eset$, and $\alf: \eset \rightarrow \lset$ a
  labelling function.
\end{definition}
For $\ae \neq \ae'$, $\alf(\ae) = \alf(\ae')$ means that $\ae$ and $\ae'$
 model different occurrences of the same action.
Intuitively, $\leq$ represents causality;
for $\ae \neq \ae'$, if $\ae \leq \ae'$
and both events occur then $\ae'$ is
caused by $\ae$.
%
In the following, we use $\emptypom$ to denote the empty lposet and
$\ae \rightarrow \ae'$ to denote that $\ae \leq \ae'$.

\begin{definition}
  Two lposets $(\eset, \leq, \alf)$ and $(\eset', \leq', \alf')$ are
  isomorphic iff there exists a bijection
  $\phi: \eset \rightarrow \eset'$ such that $\ae \leq \ae'$ iff
  $\phi(\ae) \leq' \phi(\ae')$ and $\alf = \alf' \circ \phi$.
\end{definition}

\begin{definition}
  A partially-ordered multi-set (of actions), pomset for short, is an
  isomorphism class of lposets.
\end{definition}
%
In the following, $[\eset, \leq, \alf]$ denotes the isomorphism class
of $(\eset, \leq, \alf)$, we let $\apom,\apom', \dots$ (resp.
$\aR, \aR', \dots$) range over pomsets (resp. sets of pomsets), and we
assume that any $\apom$ contains at least one lposet which will
possibly be referred to as $(\esetof \apom$,
$\leqof \apom, \alfof \apom)$.

In the following, given a natural number $n$,
$\singleton{n}$ represents the singleton $\{n\}$.
%
Also, we use $X
\uplus Y$ to represent the disjoint union of two sets $X$ and $Y$: $X
\uplus Y = (X \times \singleton{1}) \cup (Y \times \singleton{2})$.
%
Finally, given a function $f$
on $X$,
we define $f
\extension\ \singleton{n} = \{(x, n) \mapsto f(x) \stt x \in
X\}$ as the function extending $f$ to $X \times
\singleton{n}$; analogously, for a relation $R \subseteq X \times
Y$, we let $R \extension\ \singleton{n} = \{((x, n), (y,n)) \stt (x,y)
\in R\}$ be the relation extending $R$ to $(X \times \singleton{n})
\times (Y \times \singleton{n})$.

We now define two important constructions to compose pomsets
in parallel and sequentially.

%
\begin{definition}
  Let $\apom=[\eset, \leq, \alf]$ and
  $\apom'=[\eset', \leq', \alf']$ be two pomsets.
  %
  The \emph{parallel composition of $\apom$ and $\apom'$} is:
  %
  \begin{align*}
    \rpar[\apom][\apom'] \quad = \quad [\eset \uplus \eset', \ 
    (\leq \extension\ \singleton{1}) \cup 
    (\leq' \extension\ \singleton{2}),\  
    (\alf \extension\ \singleton{1}) \cup 
    (\alf' \extension\ \singleton{2})]
  \end{align*}
  For a pomset $\apom$ and a participant $\p \in \pset$, let
  $\eset_{\apom, \p} = \{\ae \in \esetof \apom \stt \subject[\alfof
  \apom(\ae)] = \p \}$ be the set of events of $\p$ in
  $\esetof \apom$.
  %
  The \emph{sequential composition of $\apom$ and $\apom'$} is:
		where
		\begin{align*}
		  \eset_{\apom, \p} = & \{\ae \in \esetof \apom \sst
		  \esbj[\alfof \apom(\ae)] = \p\}
		  \\
		  \leq_{seq}\  = &
		  \bigcup_{\p \in \pset}
								 \big((\eset_{r,\p} \times \singleton{1}) \times
								 \big\{(\ae,2) \in \eset_{r',\p} \times \singleton{2} \sst
								 \alf'(\ae) \in \lset^!\big\}\big)^\star
		  \cup
		  (\leq \extension\ \singleton{1}) \cup 
		  (\leq' \extension\ \singleton{2})
		\end{align*}
  \\
  and $\star$ is the reflexive-transitive closure.
\end{definition}
Both parallel and sequential composition preserve the causal
dependencies of its constituents $\leq$ and $\leq'$.
%
However, while there is no new dependency introduced by the parallel
composition, the sequential composition of two pomsets adds to those
in $\leq$ and $\leq'$ the dependencies among events in $\apom$ and
$\apom'$ with the same subject.
%
Basically, a causal relation is induced whenever a participant
performing a communication in $\apom$ also performs a
communication in $\apom'$.

% \begin{definition}\label{def:wellpar} Pomsets $\apom=[\eset, \leq, \alf]$ and
%   $\apom'=[\eset', \leq', \alf']$ are \emph{well-forked} if
%   \begin{align*}
%     \alf(\eset) \cap \alf'(\eset') \cap \lset^? = \emptyset
%   \end{align*}
%   We write $\wellpar[\apom][\apom']$ when $\apom$ and $\apom'$ are
%   well-forked and, for $\aG,\aG' \in \gset$, $\wellpar$ when
%   $\gsem \neq \rbot \land \gsem[\aG'] \neq \rbot \land \forall \apom
%   \in \gsem[\aG], \apom' \in \gsem[\aG'] \qst \wellpar[\apom][\apom']$
% \end{definition}

% \begin{definition}\label{def:wellseq} Pomsets $\apom=[\eset, \leq, \alf]$ and
%   $\apom'=[\eset', \leq', \alf']$ are \emph{well-sequenced} if
% \begin{align*}
% \leqof{\rseq[\apom][\apom']} \quad \supseteq \quad 
% (\{\ae \in \eset \stt \alf(\ae) \in \lset^!\} \times \singleton{1})
% \times (\{\ae \in \eset' \stt \alf'(\ae) \in \lset^?\} \times \singleton{2})
% \end{align*}
% We write $\ws[\apom][\apom']$ when $\apom$ and $\apom'$ are
% well-sequenced and, for $\aG,\aG' \in \gset$, $\ws$ when
% $\gsem \neq \rbot \land \gsem[\aG'] \neq \rbot \land \forall \apom \in \gsem[\aG],
% \apom' \in \gsem[\aG'] \qst \ws[\apom][\apom']$.
% \end{definition}

% The definition of well-branchedness relies on the notions of
% \emph{active} and \emph{passive} participants (defined
% in~\cite{tuosto:jlamp-95}) that single out those participants that
% (internally) select which branch to execute and those participants
% that have to \quo{understand} what choice was made according to the
% messages they receive, instead of internally choosing a branch.
% \begin{definition}
% Two g-choreographies $\aG$ and $\aG'$ are \emph{well-branched} when
% \begin{itemize}
% \item[($i$)] there is at most one \emph{active} participant in
%   $\gcho[]$ and
% \item[($ii$)] all the other participants of $\gcho[]$ are
%   \emph{passive}.
% \end{itemize}
% We write $\wb$ to denote that $\aG$ and $\aG'$ are well-branched.
% \end{definition}

For the sake of this paper, We restrict to well-formed~\cite{tuosto:jlamp-95} g-choreographies
for which the semantics is:
\begin{definition}[Semantics of g-choreography]
  The semantics of g-choreographies is
% by the partial map $\gsem[\_][{\nmerge[][]}] : \gset \to \parts{(\parts{\eset}   \times \parts{\eset})}$ below\footnote{We assume $\nmerge[][]$ to be understood and simply write $\gsem[\_]$.}:
\begin{align*}
  \gsem[\gempty] & = \{\emptypom\}
  \\
  \gsem[{\gint[]}] & = \{ [\big(\{\ae_1, \ae_2\},
                       \{(\ae_1,\ae_1), (\ae_2, \ae_2), (\ae_1, \ae_2)\},
                     \alf \big)] \} \text{ where } \alf : \begin{cases} \ae_1 \mapsto \aout \\ \ae_2 \mapsto \ain \end{cases}
  \\
  \gsem[{\gpar[]}] & = 
      \{\rpar[\apom][\apom'] \stt (\apom, \apom') \in {\gsem[\aG]} \times {\gsem[\aG']} \}
  \\
  \gsem[{\gseq[]}] & =
      \{\rseq[\apom][\apom'] \stt (\apom, \apom') \in {\gsem[\aG]} \times {\gsem[\aG']}\}
  \\
  \gsem[{\gcho[]}] & =  %\label{seq:cho}
      \gsem[\aG] \cup \gsem[\aG']
\end{align*}
\end{definition}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

